Blind De-anonymization Attacks using Social Networks

It is important to study the risks of publishing privacy-sensitive data. Even if sensitive identities (e.g., name, social security number) were removed and advanced data perturbation techniques were applied, several de-anonymization attacks have been proposed to re-identify individuals. However, existing attacks have some limitations: 1) they are limited in de-anonymization accuracy; 2) they require prior seed knowledge and suffer from the imprecision of such seed information. We propose a novel structure-based de-anonymization attack, which does not require the attacker to have prior information (e.g., seeds). Our attack is based on two key insights: using multi-hop neighborhood information, and optimizing the process of de-anonymization by exploiting enhanced machine learning techniques. The experimental results demonstrate that our method is robust to data perturbations and significantly outperforms the state-of-the-art de-anonymization techniques by up to $10\times$ improvement.

==> Discussion.tex <==
\section{Discussion}

{\bf Finer-grained structural information and machine learning techniques are helpful.} Previous work only utilized coarse-grained structural information. In this paper, we provide a fine-grained structural information, {$\bf nK$}-series, and a practical and novel machine learning technique, PRF-SVM, to breach users' privacy in social networks. Our new de-anonymization attack can achieve 
up to $10\times$ improvement compared with the state-of-the-art approaches. %Therefore, it is important to consider fine-grained structural information for understanding the fundamental limits of de-anonymization attacks.

{\bf Limitations:} We acknowledge that the performance of our attack may be dependent on the actual graph topologies (a limitation that is shared by most previous attacks). However, our experimental results on multiple real-world large-scale datasets suggest that our de-anonymization attack is effective in practice.

\begin{figure}[!t]
\centering{
\includegraphics[width=2in,height=1in]{./figures/shirin_overlap.eps}}

\caption{{Our approach significantly outperforms the method of Nilizadeh et al. under the partially overlapped data generated from the collaboration dataset.}}
\label{condense_overlap} %% label for entire figure

\end{figure}


